Exploring Cosmic Origins with CORE: Cosmological Parameters

We forecast the main cosmological parameter constraints achievable with the CORE space mission which is dedicated to mapping the polarisation of the Cosmic Microwave Background (CMB). CORE was recently submitted in response to ESA's fifth call for medium-sized mission proposals (M5). Here we report the results from our pre-submission study of the impact of various instrumental options, in particular the telescope size and sensitivity level, and review the great, transformative potential of the mission as proposed. Specifically, we assess the impact on a broad range of fundamental parameters of our Universe as a function of the expected CMB characteristics, with other papers in the series focusing on controlling astrophysical and instrumental residual systematics. In this paper, we assume that only a few central CORE frequency channels are usable for our purpose, all others being devoted to the cleaning of astrophysical contaminants. On the theoretical side, we assume LCDM as our general framework and quantify the improvement provided by CORE over the current constraints from the Planck 2015 release. We also study the joint sensitivity of CORE and of future Baryon Acoustic Oscillation and Large Scale Structure experiments like DESI and Euclid. Specific constraints on the physics of inflation are presented in another paper of the series. In addition to the six parameters of the base LCDM, which describe the matter content of a spatially flat universe with adiabatic and scalar primordial fluctuations from inflation, we derive the precision achievable on parameters like those describing curvature, neutrino physics, extra light relics, primordial helium abundance, dark matter annihilation, recombination physics, variation of fundamental constants, dark energy, modified gravity, reionization and cosmic birefringence. (ABRIDGED)

==> section_delensing.tex <==
\section{Delensing\label{sec:delensing}}

\emph{This part has been written by Josquin Errard. We should keep it only if we use his delensing noise spectrum somewhere.}\\
Section~\ref{} describes how large scale structures induce gravitational lensing on CMB maps and, in particular, in polarization. Characterizing this effect gives an opportunity to study the gravitational potential along the line-of-sight, allowing us to constrain the cosmological parameters involved in the evolution of matter distribution, e.g. neutrino mass or dark energy properties.

\begin{figure}
	\centering
		\includegraphics[width=12cm]{figures/FGspectra_Errard2016.pdf}
	\caption{Comparison of diffuse astrophysical foregrounds amplitudes with cosmological signals, in particular the primordial and lensed $B$-modes. The sensitivity to primordial signal is limited by galactic emissions and gravitational lensing (from~\cite{Errard2016}).}
\label{fig:FGspectra}
\end{figure}

However, CMB lensing can also be considered as a nuisance in the quest for primordial gravitational waves.
In fact, lensing mixes the $E$ and $B$ polarization modes \cite{Lewis&Challinor 2006}, and since the primordial $B$-modes signal only arises from primordial tensor perturbations which are much smaller than the scalar ones (generating $E$ polarization), lensing transfers a significant amount of $E$ into $B$ polarization. The amplitude of these so-called lensed $B$ modes peaks around a multipole $\ell\sim1000$ and, with $r<0.07$ \cite{BKP2015?}, is always larger than the primordial signal on scales smaller than the reionization bump. 
Lensing is therefore, after the diffuse astrophysical foregrounds, the second largest contaminant in the search for $r$, cf. Fig.~\ref{fig:FGspectra}.

Techniques have been proposed to \emph{delens} the CMB polarization maps
%\citep{2015PhRvD..92d3005S, 2015ApJ...807..166S,2007PhRvD..76l3009M,2004PhRvD..69d3005S,2002PhRvL..89a1304K,2002PhRvL..89a1303K,2012JCAP...06..014S}
, i.e. in order to reduce the extra \emph{variance} induced by lensing. 
Delensing proposes to remove the lensing induced signal from the observed CMB, and that requires an estimate of the unlensed CMB as well as the matter distribution. The latter can be obtained either from external surveys (cosmic shear, galaxy catalogs, 21cm, CIB) or from the CMB lensing estimate itself (using e.g. quadratic or max-likelihood estimators). The former can be obtained at first order from observed $E$-modes, since lensing is only a small correction. Note that when delensing is performed using the internal CMB lensing estimate, its accuracy can be improved by iterating over the delensing step, replacing the observed CMB maps with the delensed one from a previous step. 

The performance of delensing would depend on the experimental characteristics and on the choice for the matter distribution estimator. Detailed analysis of the delensing efficiency and its propagation to limits on $r$ is discussed in~\cite{Errard2016}. 
In addition to improving the sensitivity to $r$, delensing could also simplify the analysis of a joint lensing and CMB constraint on neutrino masses~\cite{2003PhRvL..91x1301K}. Similarly, constraints on $N_{\rm eff}$ have been shown to improve significantly after delensing the observed $E$-modes~\cite{CMB-S4-Science-Book}.

\begin{figure}
	\centering
		\includegraphics[width=7.5cm]{figures/alpha_vs_uKarcmin_errard16.pdf}~\includegraphics[width=7.5cm]{figures/sigma_r_vs_fsky_uKarcmin_errard16.pdf}
	\caption{\textit{Left panel:} $\alpha$, the delensing improvement, shown as a function of the noise in the CMB map after component separation. $\alpha$ is defined as the ratio of the integrated powers between the delensed and lensed B-modes, around the recombination bump ($20\leq\ell\leq200$). The delensing improvement is shown here using an iterative delensing based on the observation of $E$ and $B$-modes (dark orange), using CIB information (light orange) and using a futuristic large scale structure survey (dark red). The result assumes FWHM=$3'$ and a multipole range of $\sqrt{ 2\pi / f_{\rm sky}} \leq \ell \leq 3000$. \textit{Right panel:} One-sigma limit on $r=0$, $\sigma(r=0)$, as a function of both the noise in the CMB map and the observed fraction of the sky. Grey (respectively black) contours correspond to the no delensing (respectively iterative CMB delensing) case. No foreground residuals are taken into account in this result. Figures taken from~\cite{Errard2016}. }
\label{fig:sigma_r_mnu_vs_fsky_uKarcmin_Errard2016}
\end{figure}

The left panel of Fig.~\ref{fig:sigma_r_mnu_vs_fsky_uKarcmin_Errard2016} shows the delensing factor $\alpha$, introduced in~\cite{Errard2016}, as a function of the post-component-separation sensitivity of a CMB experiment with a Gaussian beam with full-width at half-maximum (FWHM) of $3'$. Plotted are three delensing methods considered in~\cite{Errard2016}: iterative delensing using the CMB polarization, and via cross-correlation with the CIB or a large scale structure survey. The first point to note is that delensing exploiting the correlation with large scale structures only slightly outperforms the delensing with CIB, even though the latter makes use of existing Planck data products~\cite{2015PhRvD..92d3005S}. Moreover, for both cross-correlation methods the sensitivity of the CMB instrument does not matter in the regime $\leq 5-10\ \mu$K-arcmin, as the $E$-mode observations are largely cosmic-variance limited for these sensitivities. Iterative delensing using CMB polarization becomes more effective than the cross-correlation techniques when the post-component separation noise level drops below $\sim\,3\ \mu$K-arcmin. Note that other quadratic combinations of CMB fields --- and, indeed, their minimum-variance combination~\cite{2002ApJ...574..566H} --- will outperform the ``$EBEB$'' estimator considered here in the high-noise regime.
This result is a consequence of $N_\ell^{\phi\phi}$ which continues to decrease as the instrumental sensitivity increases, in the framework of iterative delensing~\cite{2004PhRvD..69d3005S}.
Note also that the curves become thicker as the noise level decreases. This effect is due to varying the area of sky to which the experiment has access (sky fractions considered here span the range 1--100\%). Larger-scale experiments have access to more multipoles (we assume $\ell_{\rm min} \propto f_{\rm sky}^{-1/2}$) which allows for improved iterative delensing at low noise levels.

We do not show here the dependence of $\alpha$ upon the instrumental angular resolution. Yet, it is important to note that un-observed $E$-modes between $100 \leq \ell \leq 1000$ will significantly degrade the reconstruction of lensed $B$-modes and therefore their subtraction. In addition, for a given CMB map sensitivity, the reconstruction of the lensing potential will be optimized by looking at rather high-$\ell$ in all CMB power spectra.

==> table_example.tex <==
\begin{table}[h]
\begin{center}\footnotesize
\scalebox{0.87}{\begin{tabular}{|c||c|c|c|c|c|}
\hline
\hline 
Parameter         & Planck + lensing & LiteCORE 80, TEP& LiteCORE120, TEP& CORE-M5, TEP& COrE+, TEP  \\            
%notice that we use COrE+
\hline
$w$ &      $-1.42\,_{-0.45}^{+0.26}$&      $-1.06\,_{-0.11}^{+0.19}$& $-1.05\,_{-0.10}^{+0.16}$& $ -1.04\,_{-0.09}^{+0.15}$&$ -1.04\,_{-0.09}^{+0.14}$ \\
$\Omega_bh^2$ &      $0.02225\pm0.00016$&      $0.022186\pm0.000056$& $0.022183\pm0.000041$& $ 0.022182\pm0.000039$&$ 0.022183\pm0.000034$ \\
$\Omega_ch^2$ &      $0.1192\pm0.0014$&      $0.12036\pm0.00061$& $0.12040\pm0.00055$& $ 0.12041\pm0.00051$&$ 0.12039\pm0.00047$ \\
$100\theta_{MC}$ &      $1.04087\pm0.00033$&      $1.04070\pm0.00010$& $1.040698\pm0.000088$& $ 1.040695\pm0.000083$&$ 1.040698\pm0.000078$ \\
$\tau$ &      $0.055\pm 0.015$&      $0.0597\,_{-0.0022}^{+0.0019}$& $0.0596\pm0.0020$& $ 0.0597\,_{-0.0021}^{+0.0019}$&$ 0.0597\,_{-0.0022}^{+0.0019}$ \\
$n_s$ &      $0.9653\pm0.0047$&      $0.9621\pm0.0020$& $0.9621\pm0.0018$& $ 0.9621\pm0.0018$&$ 0.9621\pm0.0017$ \\
$ln(10^{10}A_s)$ &      $3.042\pm0.028$&      $3.0558\pm0.0040$& $3.0557\,_{-0.0044}^{+0.0039}$& $ 3.0560\,_{-0.0042}^{+0.0037}$&$ 3.0558\,_{-0.0042}^{+0.0038}$ \\
\hline
%notice the line for the derived parameters to be listed below
$H_0$ &      $>75.6$&      $69.0\,_{-6.1}^{+3.1}$& $68.5\,_{-5.1}^{+2.9}$& $ 68.1\,_{-4.6}^{+2.8}$&$ 68.3\,_{-4.4}^{+2.7}$ \\
$\sigma_8$ &      $0.93\,_{-0.07}^{+0.12}$&      $0.834\,_{-0.051}^{+0.028}$& $0.830\,_{-0.043}^{+0.026}$& $ 0.827\,_{-0.039}^{+0.025}$&$ 0.828\,_{-0.037}^{+0.024}$ \\
\hline
\end{tabular}}
\end{center}
\caption{$68\%$~CL constraints on cosmological parameters in the $\Lambda$CDM + w model from the
Planck+Lensing real dataset (see \cite{planck2015}) and different CORE experimental specifications.}
\label{tab:params_w}
\end{table}
